Planarity and dimension II

The dimension of a poset $P$ is the minimum positive integer $d$ such that $P$ is an induced subposet of $\mathbb{R}^d$ equipped with the product order. We give a constant-factor polynomial-time approximation algorithm for computing dimension in the class of posets with a planar (Hasse) diagram. While computing the dimension of a poset is NP-hard in general, the computational complexity of the problem for planar posets remains open. The algorithmic result is driven by a structural understanding of the canonical obstruction to small dimension: standard examples. A longstanding problem, originating in the early 1980s, asked whether every poset with a planar diagram has dimension bounded by a function of the maximum order of a standard example that it contains. In the first paper of the series, we have resolved the problem in a more general setting of posets with planar cover graphs by establishing a polynomial bound. We prove a stronger bound in the original setting, namely, for every poset $P$ with a planar diagram $\mathrm{dim}(P) \leq 96\mathrm{se}(P)+672$, where $\mathrm{dim}(P)$ denotes the dimension of $P$ and $\mathrm{se}(P)$ denotes the maximum order of a standard example contained in $P$.

==> style.table-of-contents.tex <==
% https://tex.stackexchange.com/questions/633286/how-to-add-dots-to-ams-table-of-contents
\usepackage{xpatch}
\makeatletter   
\xpatchcmd{\@tocline}
{\hfil\hbox to\@pnumwidth{\@tocpagenum{#7}}\par}
{\ifnum#1<2\hfill\else\dotfill\fi\hbox to\@pnumwidth{\@tocpagenum{#7}}\par}
{}{}
\makeatother    
% *******************************************   

\makeatletter
\def\l@section{\vspace*{5pt}\bfseries\@tocline{1}{0pt}{0pc}{4pc}{}}
\def\l@subsection{\mdseries\@tocline{2}{0pt}{4pc}{6pc}{}}
\def\l@subsubsection{\mdseries\@tocline{3}{0pt}{8pc}{8pc}{}}
\makeatother


